Adaptive Optics Observations of the Galactic Center Young Stars

Adaptive Optics observations have dramatically improved the quality and versatility of high angular resolution measurements of the center of our Galaxy. In this paper, we quantify the quality of our Adaptive Optics observations and report on the astrometric precision for the young stellar population that appears to reside in a stellar disk structure in the central parsec. We show that with our improved astrometry and a 16 year baseline, including 10 years of speckle and 6 years of laser guide star AO imaging, we reliably detect accelerations in the plane of the sky as small as 70 microarcsec/yr/yr (~2.5 km/s/yr) and out to a projected radius from the supermassive black hole of 1.5" (~0.06 pc). With an increase in sensitivity to accelerations by a factor of ~6 over our previous efforts, we are able to directly probe the kinematic structure of the young stellar disk, which appears to have an inner radius of 0.8". We find that candidate disk members are on eccentric orbits, with a mean eccentricity of < e > = 0.30 +/- 0.07. Such eccentricities cannot be explained by the relaxation of a circular disk with a normal initial mass function, which suggests the existence of a top-heavy IMF or formation in an initially eccentric disk.

==> jlu_macros.tex <==
\newcommand{\msun}{M$_{\odot}$\,}
\newcommand{\Ms}{M$_s$}
\newcommand{\Lp}{L'}
\newcommand{\Kp}{K'}
\newcommand{\Hp}{H}

% matthew macros
\def\procspie{Proc. SPIE}
\def\newar{NewAR}
\def\pasj{PASJ}
\def\newblock{\hskip .11em plus .33em minus .07em}
%\newcommand\figcaption{\caption}
%\newcommand\singlespace{\renewcommand\baselinestretch{1.0}}
\newcommand\defaultspace{\renewcommand\baselinestretch{@spacing}}
%\newcommand{\figcaption}[2]{\singlespace \caption[#1]{#2} \defaultspace}
\newcommand\ts{\thinspace}

% macros from caer
%\newcommand{\micron}{$\mu m$ }
%\newcommand{\arcsec}[0]{''}
\def\sun{\hbox{$\odot$}}
\def\earth{\hbox{$\oplus$}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\arcdeg{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}}
\def\farcs{\hbox{\kern 0.13ex.\kern -0.95ex%
\raisebox{.9ex}{\scriptsize$\prime\prime$}\kern -0.1ex}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\micron{\hbox{$\mu$m}}
\def\kms{km s${}^{-1}$}
\newcommand{\Ha}{H$\alpha$ }
\newcommand{\brg}{Br $\gamma$ }
\newcommand{\obs}{\it data}
\newcommand{\nsf}{NSFCAM}
\newcommand{\osc}{OSCIR}
\newcommand{\lw}{LWS}
\newcommand{\sig}{$\pm$}
\newcommand{\ulim}{$>$}
\newcommand{\av}{$A_{v}$\,}
\newcommand{\kl}{$K-L$\,}
\newcommand{\kn}{$K-N$\,}
\newcommand{\knobs}{$K-[N]$\,}
\newcommand{\lncolor}{$L-N$\,}
\newcommand{\sigm}{$\sigma$\,}
\newcommand{\app}{$\sim$}

% \input {mymacros}                         % personal LaTeX macros
% from amy
\def\sun{\hbox{$\odot$}}
\def\apj{ApJ}
\def\apjl{ApJL}
\def\aj{AJ}
\def\nat{Nature}
\def\araa{ARAA}
\def\aaps{A\&AS}
\def\apjs{ApJS}
\def\it{}
\def\mnras{MNRAS}
\def\aap{AAP}
\def\na{New Astronomy}
\def\nar{New Astron. Rev.}
\def\pasp{PASP}
\def\prd{Phys. Rev. D}
\def\physrep{Phys. Rep.}
\def\earth{\hbox{$\oplus$}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\arcdeg{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{.\kern -0.7ex\raisebox{.9ex}{\scriptsize$\prime$}}}
\def\farcs{\hbox{\kern 0.13ex.\kern -0.95ex%
\raisebox{.9ex}{\scriptsize$\prime\prime$}\kern -0.1ex}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\kms{km s${}^{-1}$}
\def\ab{$\sim$}
\def\degr{^{\circ}}
\def\cd{CoD $-$33$\deg$7795 }
\def\Ha{H$\alpha$ }
\def\ha{H$\alpha$ }
\def\arcsec{''}
\def\sub{$\circ$}
\def\deg{\hbox{$^\circ$}}
\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sq{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\onehalf{\hbox{$\,^1\!/_2$}}        % Common fractions with solidus
\def\onethird{\hbox{$\,^1\!/_3$}}
\def\twothirds{\hbox{$\,^2\!/_3$}}
\def\onequarter{\hbox{$\,^1\!/_4$}}
\def\threequarters{\hbox{$\,^3\!/_4$}}
%\def\plotone{\includegraphics}

%\def\thefigure{\@arabic\c@figure}%
%\def\thetable{\@arabic\c@table}%
%\def\theplate{\@arabic\c@plate}%
\def\fnum@figure{{\rmfamily Fig.\space\thefigure.---}}%
\def\fnum@table{{\rmfamily Table \thetable:}}%
\def\fnum@plate{{\bfseries Plate \theplate.}}%
\def\fps@figure{bp}%
\def\fps@table{bp}%
\def\fps@plate{bp}%
\def\eps@scaling{1.0}%
%\newcommand\epsscale[1]{\gdef\eps@scaling{#1}}%
%\newcommand\plotone[1]{%
% \typeout{Plotone included the file #1}
% \centering
% \leavevmode
% \includegraphics[width={\eps@scaling\columnwidth}]{#1}%
%}%
%\newcommand\plottwo[2]{{%
% \typeout{Plottwo included the files #1 #2}
% \centering
% \leavevmode
% \columnwidth=.45\columnwidth
% \includegraphics[width={\eps@scaling\columnwidth}]{#1}%
% \hfil
% \includegraphics[width={\eps@scaling\columnwidth}]{#2}%
%}}%

